Scalable Second-Order Optimization Algorithms for Minimizing Low-rank Functions

We present a random-subspace variant of cubic regularization algorithm that chooses the size of the subspace adaptively, based on the rank of the projected second derivative matrix. Iteratively, our variant only requires access to (small-dimensional) projections of first- and second-order problem derivatives and calculates a reduced step inexpensively. The ensuing method maintains the optimal global rate of convergence of (full-dimensional) cubic regularization, while showing improved scalability both theoretically and numerically, particularly when applied to low-rank functions. When applied to the latter, our algorithm naturally adapts the subspace size to the true rank of the function, without knowing it a priori.

==> preamblesAndMacros.tex <==
% Warning filter
\usepackage{silence}
\WarningFilter[pdftoc]{hyperref}{Token not allowed in a PDF string}

% packages
    \usepackage[utf8]{inputenc}
    \usepackage[T1]{fontenc}
    \usepackage{siunitx}
    \usepackage{colonequals}
    \usepackage[super]{nth}
    \usepackage{algorithm}
    \usepackage{amsmath}
    \usepackage{amsthm}
    \usepackage{amssymb}
    \usepackage{tikz}
    \usepackage{url}
    \usepackage{float}
    \usepackage{tabularx}
    \usepackage{pbox}
    \usepackage{tabulary}
    \usepackage{breqn}
    \usepackage{longtable}
    \usepackage{mdframed}
    \usepackage{booktabs}

    % Figures
    \usepackage{graphicx}
    \graphicspath{{./images/}{./}}

    \usepackage{wrapfig}
    \usepackage[font={small}]{caption}
    \usepackage{enumitem}
    \usepackage{physics}
    \usepackage{lipsum}
    \usepackage{mwe}
    \usepackage{breqn}
    \usepackage[noend]{algpseudocode}
    \usepackage{subcaption}
    \usepackage{graphicx}
    \usepackage{enumitem}
    \usepackage{bm}
    \usepackage{textcmds}

    %Appendix numbering
    \usepackage{apptools}
    \AtAppendix{\counterwithin{lemma}{section}}
    \AtAppendix{\counterwithin{remark}{section}}
    
    % Reference Style
    \usepackage{hyperref}
    \hypersetup{
        colorlinks,
            citecolor=black,
        filecolor=black,
        linkcolor=black,
        urlcolor=black
    } 
    

% Auto-refs
\newcommand{\algautorefname}{Algorithm}
\newcommand{\claimautorefname}{Claim}
\renewcommand{\theoremautorefname}{Theorem}
\newcommand{\lemmaautorefname}{Lemma}
\newcommand{\remarkautorefname}{Remark}
\newcommand{\corollaryautorefname}{Corollary}
\newcommand{\conjectureutorefname}{Conjecture}
\newcommand{\observationautorefname}{Observation}
\newcommand{\myQuoteautorefname}{Quote}
\newcommand{\factautorefname}{Fact}
\newcommand{\definitionautorefname}{Definition}
\newcommand{\assumptionautorefname}{Assumption}
\newcommand{\exampleautorefname}{Example}
\newcommand{\algorithmautorefname}{Algorithm}
\newcommand{\proofautorefname}{Proof}


% New Environments

\newtheorem{corollary}{Corollary}
\newtheorem{claim}{Claim}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{corallary}{Corollary}
\newtheorem{conjecture}{Conjecture}
\newtheorem*{observation}{Observation}
\newtheorem*{myQuote}{Quote}
\newtheorem{fact}{Fact}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\newtheorem{example}{Example}
\newtheorem{alg}{Algorithm}

% Environment numbering
\numberwithin{equation}{section} % use section numbering
\numberwithin{lemma}{section} % use section numbering
\numberwithin{theorem}{section} % use section numbering
\numberwithin{definition}{section} % use section numbering
\numberwithin{corollary}{section} % use section numbering

% Maths Operator
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

% Maths Macro
\newcommand{\LH}{L_H}
\newcommand{\kappaS}{\kappa_S}
\newcommand{\Bepsilon}{\bar{\epsilon}}
\newcommand{\logOneOverDeltaS}{\log \bracket{\frac{1}{\deltaS}}}
\newcommand{\chernoffLowerExponentialCubic}{e^{-\frac{\delta_1^2}{2} (\frac{7}{8}) N}}
\newcommand{\nPreFactorTRCubic}{\left[\frac{7}{8}(1-\delta_1) - 1 + \frac{c}{(c+1)^2} \right]^{-1}}
\newcommand{\deltaSThreeExpression}{\pow{e}{-\frac{l(\epSTwo)^2}{C_l} + r +1 }}
\newcommand{\newL}{\tau_{\alpha}}
\newcommand{\mRLEpsKappa}{m(\epsOne, r, l, \kappa_H)}
% \newcommand{\epsOne}{\epsilon_1}
\newcommand{\epsOne}{\epS}
\newcommand{\nThreeEpH}{N_{\epH}^{(3)}}
\newcommand{\hTwoEpsHAlphaZeroGammaOneCL}{h_2(\epH,\alphaZeroGammaOneCL)}
\newcommand{\nTwoEpsH}{N_{\epH}^{(2)}}
\newcommand{\hOneEpsHAlphaZeroGammaOneCL}{h_1(\epH, \alphaZeroGammaOneCL)}
\newcommand{\alphaZeroGammaOneCL}{\alpha_0\gammaOne^{c+l}}
\newcommand{\IterKTrueandSuccssfulWithAlphaKGeq}[1]{
\substack{ \text{Iteration $k$ is true and successful} \\ 
\text{with $\alphaK \geq #1$}}}
\newcommand{\epH}{\epsilon_{H}}
\newcommand{\epsHalf}{\epsilon^{\frac{1}{2} }  }
\newcommand{\oneMinusEpSHalf}{(1-\epS)^{\frac{1}{2}}}
\newcommand{\NsKTSKHat}{\normTwo{S_k^T \sKHat}}
\newcommand{\deltaSThree}{\deltaS^{(3)}}
\newcommand{\ntsAlphaC}{N_{TS, \underline{\alpha_c}}}
\newcommand{\fZeroMinusfStarOverH}{\frac{f(x_0) - f^*}{h(\epsilon, \alphaZero\gammaOne^{c+\newL}
)}}
\newcommand{\ntsAlphaZeroGammaOneCL}{N_{TS, \underline{\alphaZero \gammaOne^{c+\newL}}}}
\newcommand{\fun}[2]{#1\bracket{#2}}
\newcommand{\pow}[2]{#1^{#2}}
\newcommand{\impliesSince}[1]{\overset{#1}{\implies}}
\newcommand{\hK}{\grad^2 f(x_k)}
\newcommand{\qK}[1]{q_k \bracket{#1}}
\newcommand{\qKHat}[1]{\hat{q}_k \bracket{#1}}
\newcommand{\epSOne}{\epsilon_S^{(1)}}
\newcommand{\epSTwo}{\epsilon_S^{(2)}}
\newcommand{\MK}{M_k}
\newcommand{\hessFK}{\grad^2 f(x_k)}
\newcommand{\SK}{S_k}
\newcommand{\oneMinusEpSOne}{1 - \epSOne}
\newcommand{\oneMinusEpSTwo}{1 - \epSTwo}

\newcommand{\sqrtFrac}[2]{\sqrt{\frac{#1}{#2}}}
\newcommand{\gDeltaSDeltaOne}{g(\deltaS, \deltaOne)}
\newcommand{\mathOmega}[1]{\Omega \left( #1 \right) }
\newcommand{\mathO}[1]{\mathcal{O}\left( #1\right)}
\newcommand{\ra}{\rangle}
\newcommand{\la}{\langle}
\newcommand{\norms}[1]{\|#1\|_2^2}
\newcommand{\Z}{\mathbb{Z}} 
\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\dotp}[2]{\langle #1, #2 \rangle}
\newcommand{\alphaLow}{\alpha_{low}}
\newcommand{\nEps}{N_{\epsilon}}
\newcommand{\oneOverGammaOneC}{\frac{1}{\gamma_1^c}}
\newcommand{\nt}{N_T}
\newcommand{\nts}{N_{TS}}
\newcommand{\ns}{N_S}
\newcommand{\nuMe}{N_U}
\newcommand{\ntu}{N_{TU}}
\newcommand{\ntAlphaUpper}{N_{T, \overline{\alphaLowOne}}}
\newcommand{\nsAlphaUpper}{N_{S, \overline{\alphaLowOne}}}
\newcommand{\ntAlphaLower}{N_{T, \underline{\alphaLowOne}}}
\newcommand{\ntsAlphaLower}{N_{TS, \underline{\alphaLowOne}}}
\newcommand{\ntuAlphaLower}{N_{TU, \underline{\alphaLowOne}}}
\newcommand{\nuAlphaLower}{N_{U, \underline{\alphaLowOne}}}
\newcommand{\nsGammaAlpha}{N_{S, \underline{ \gamma_1^{c}\alphaLowOne}}}
\newcommand{\ntsGammaCAlpha}{N_{TS, \underline{ \gamma_1^c \alphaLowOne}}}
\newcommand{\nfsGammaAlpha}{N_{FS, \underline{ \gamma_1^c \alphaLowOne}}}
\newcommand{\nf}{N_F}
\newcommand{\etaHAlphaK}{h \left( \epsilon, \alpha_k \right)}
\newcommand{\etaHAlphaLow}{h \left(  \epsilon, \alphaLow \right)}
\newcommand{\etaHAlphaMin}{h \left(  \epsilon, \alphaMin \right)}
\newcommand{\etaHAlphaLowGammaC}{h \left( \epsilon, \gamma_1^c \alphaMin \right)}
\newcommand{\ntsUpper}{\frac{f(x_0)-f^*}{\etaHAlphaLow}}
\newcommand{\ntsUpperGammaC}{\frac{f(x_0)-f^*}{\etaHAlphaLowGammaC}}
\newcommand{\logOneOverGammaOne}{\log(1/\gamma_1)}
\newcommand{\logAlphaZeroOverAlphaLow}{\log\left(\frac{\alpha_{0}}{\alphaMin}\right)}
\newcommand{\nuUpper}{\frac{C_1 + C_2 N}{1 + C_2}}
\newcommand{\logGammaTwoOverGammaOne}{\log(\gamma_2/\gamma_1)}
\newcommand{\tCOne}{\newL}
\newcommand{\tCTwo}{c}
\newcommand{\logAlphaLowOverAlphaZeroBaseGamma}{\log_{\gamma_1} (\alphaMin/\alpha_0)}
\newcommand{\nuUpperT}{\frac{\tCOne + \tCTwo N}{1 + \tCTwo}}
\newcommand{\expectation}[1]{\E \left[ #1 \right]}
\newcommand{\sumTk}{\sum_{k=0}^{N-1} T_k}
\newcommand{\eToMinusLambdaMinusOne}{e^{-\lambda}-1}
\newcommand{\oneMinusDeltaS}{1-\delta_S}
\newcommand{\conditionalE}[2]{\E \left[ #1 | #2 \right]}
\newcommand{\eToMinusLambdaSumTk}{e^{-\lambda \sumTk }}
\newcommand{\eToMinusLambdaSumTkNMinusTwo}{e^{-\lambda \sumTkToNMinusTwo }}
\newcommand{\exponentialMomentUpperTotal}{\left[ e^{( \eToMinusLambdaMinusOne)(\oneMinusDeltaS)}\right]^N}
\newcommand{\exponentialMomentUpper}{ e^{( \eToMinusLambdaMinusOne)(\oneMinusDeltaS)}}
\newcommand{\eToMinusLambda}[1]{e^{-\lambda #1}}
\newcommand{\conditionalP}[2]{\P \left[ #1 | #2 \right]}
\newcommand{\sumTkToNMinusTwo}{\sum_{k=0}^{N-2}T_k}
\newcommand{\SZeroDotsToXNMinusOne}{T_0, T_1, \dots, T_{N-2}, x_{N-1}}
\newcommand{\deltaOneComplicated}{-\delta_1 - (1-\delta_1) \log(1-\delta_1) }
\newcommand{\chernoffLowerExponential}{e^{-\frac{\delta_1^2}{2} (1-\delta_S) N}}
\newcommand{\chernoffLower}{1 - \chernoffLowerExponential }
\newcommand{\nPreFactor}{\left[(1-\delta_S)(1-\delta_1) - \frac{C_2}{1+C_2} \right]^{-1}}
\newcommand{\nPreFactorTR}{\left[(1-\delta_S)(1-\delta_1) - 1 + \frac{c}{(c+1)^2} \right]^{-1}}
\newcommand{\betaK}{\beta_k}
\newcommand{\kStartOne}{k_{\small{start}}^{(1)}}
\newcommand{\kEndOne}{k_{\small{end}}^{(1)}}
\newcommand{\aOne}{A^{(1)}}
\newcommand{\closedInterval}[2]{\left[ #1, #2 \right]}
\newcommand{\twoCases}[4]{         \begin{cases}
             #1, & #2 \\
             #3, & #4.
        \end{cases} }
\newcommand{\closedOpenInterval}[2]{\left[ #1, #2 \right)}
\newcommand{\openClosedInterval}[2]{\left( #1, #2\right]}
\newcommand{\openInterval}[2]{\left( #1, #2\right)}
\newcommand{\mOneOne}{M_1^{(1)}}
\newcommand{\mTwoOne}{M_2^{(1)}}
\newcommand{\nOneOne}{n_1^{(1)}}
\newcommand{\nTwoOne}{n_2^{(1)}}
\newcommand{\kInStartEndOne}{k \in \openInterval{\kStartOne}{\kEndOne}}
\newcommand{\bOne}{B^{(1)}}
\newcommand{\kStartTwo}{k_{\small{start}}^{(2)}}
\newcommand{\kEndTwo}{k_{\small{end}}^{(2)}}
\newcommand{\kStartThree}{k_{\small{start}}^{(3)}}
\newcommand{\kStartI}{k_{\small{start}}^{(i)}}
\newcommand{\kStartIPlusOne}{k_{\small{start}}^{(i+1)}}
\newcommand{\kEndI}{k_{\small{end}}^{(i)}}
\newcommand{\aTwo}{A^{(2)}}
\newcommand{\mOneTwo}{M_1^{(2)}}
\newcommand{\mTwoTwo}{M_2^{(2)}}
\newcommand{\nOneTwo}{n_1^{(2)}}
\newcommand{\nTwoTwo}{n_2^{(2)}}
\newcommand{\kInStartEndTwo}{k \in \closedOpenInterval{\kStartTwo}{\kEndTwo}}
\newcommand{\bTwo}{B^{(2)}}
\newcommand{\logGammaTwoAlphaLowOverAlphaZero}{\log\left( \gamma_2 \alphaLow/\alpha_0\right)}
\newcommand{\kBar}{\overline{k}}
\newcommand{\onePlusTCTwo}{1+ \tCTwo}
\newcommand{\fZeroMinusfStar}{f_0 - f^*}
\newcommand{\sHat}{\hat{s}}
\newcommand{\mKHat}[1]{\hat{m}_k\left( #1\right)}
\newcommand{\xK}{x_k}
\newcommand{\xKPlusOne}{x_{k+1}}
\newcommand{\sK}{s_k}
\newcommand{\normTwo}[1]{\left\lVert#1\right\rVert_2}
\newcommand{\gradFK}{\grad f(\xK)}
\newcommand{\DOneOverNMinusDTwo}{\frac{D_1}{N-D_2}}
\newcommand{\qInverseOfDOneOverNMinusDTwo}{q^{-1} \left( \DOneOverNMinusDTwo\right)}
\newcommand{\minGradient}[1]{\min_{k\leq #1} \normTwo{\gradFK}}
\newcommand{\minGradientN}{\minGradient{N}}
\newcommand{\nUpperThmOne}{\nPreFactor \left[ \ntsUpper + \frac{C_1}{1+C_2}\right]}
\newcommand{\DOneOverQPlusDTwo}{\frac{D_1}{q(\epsilon)}+D_2}
\newcommand{\DOneOverHPlusDTwo}{\frac{D_1}{h(\epsilon, \alphaLow)}+D_2}
\newcommand{\logOneOverDelta}{\log\left( \frac{1}{\delta}\right)}
\newcommand{\eToMinusDThreeN}{e^{-D_3 N}}
\newcommand{\gammaOneC}{\gamma_1^c}
\newcommand{\hatNOneOne}{\hat{n}_1^{(1)}}
\newcommand{\hatNOneTwo}{\hat{n}_2^{(1)}}
\newcommand{\fK}{f(x_k)}
\newcommand{\innerProduct}[2]{\langle #1, #2 \rangle}
\newcommand{\sKGradFK}{S_k \gradFK}
\newcommand{\sKBKSKT}{S_k B_k S_k^T}
\newcommand{\rLTimesD}{\R^{l\times d}}
\newcommand{\fKPlusOne}{f(x_k + s_k)}
\newcommand{\epS}{\epsilon_S}
\newcommand{\sMax}{S_{\small{max}}}
\newcommand{\alphaMax}{\alpha_{\small{max}}}
\newcommand{\alphaK}{\alpha_k}
\newcommand{\hBar}{\bar{h}}
\newcommand{\deltaSOne}{\delta_S^{(1)}}
\newcommand{\deltaSTwo}{\delta_S^{(2)}}
\newcommand{\aKOne}{A_k^{(1)}}
\newcommand{\aKTwo}{A_k^{(2)}}
\newcommand{\intersect}{\cap}
\newcommand{\barXK}{\bar{x}_k}
\newcommand{\probabilityGivenXK}[1]{\probability{#1 | x_k = \barXK}}
\newcommand{\aKOneIntersectaKTwo}{\aKOne \intersect \aKTwo}
\renewcommand{\complement}[1]{\left( #1\right)^c}
\newcommand{\oneMiusEpsSToHalf}{\left( 1-\epS\right)^{1/2}}
\newcommand{\gammaTwoAlphaMaxAlphaLowConditions}{    
    $\gamma_2 = \oneOverGammaOneC$, $\alpha_{max} = \frac{\alpha_0}{\gamma_1^p} , \alphaLow = \alpha_0 \gamma^l$ for some $c,p,l\in \N^+$}
\renewcommand{\abs}[1]{\lvert #1\rvert}
\newcommand{\kLeqNsuchthat}{k\leq N:}
\newcommand{\ntDef}{\abs{\set{\kLeqNsuchthat \text{iteration $k$ is successful}}}}
\newcommand{\definedAs}{defined as}
\newcommand{\alphaKPlusOne}{\alpha_{k+1}}
\newcommand{\gammaOne}{\gamma_1}
\newcommand{\gammaTwo}{\gamma_2}
\newcommand{\logMe}[1]{\log \left( #1 \right)}
\newcommand{\alphaZero}{\alpha_0}
\newcommand{\alphaMin}{\alpha_{\small{min}}}
\newcommand{\floor}[1]{\left \lfloor{#1}\right \rfloor }
\newcommand{\ceil}[1]{\left \lceil{#1}\right \rceil}
\newcommand{\logBaseGammaOne}[1]{\log_{\gammaOne}\left( #1\right)}
\newcommand{\minMe}[2]{\min \set{#1, #2}}
\newcommand{\alphaLowOne}{\alphaMin}
\newcommand{\pOneDef}{\frac{\log(\gammaTwo\alphaMin/\alphaZero)}{\logGammaTwoOverGammaOne}}
\newcommand{\pZeroDef}{ \frac{\logOneOverGammaOne}{\logGammaTwoOverGammaOne}}
\newcommand{\alphaMaxDef}{\frac{\alphaZero}{\gamma_1^p}}
\newcommand{\gammaTwoExpression}{ \frac{1}{\gamma_1^c}}
\newcommand{\betaKPlusOne}{\beta_{k+1}}
\newcommand\muAOneHashing{C_1 \sqrt{C_2} \sqrt{\epsilon}  \min \left\{\frac{\log(E/ (C_2 \epsilon))}{4r + \log(1/\delta)}, \sqrt{\frac{\log(E)}{4r + \log(1/\delta)}} \right\} }
\newcommand\logDeltaI{\log(1/\delta)}
\newcommand\fourRplusLog{\left[ 4r + \logDeltaI\right]}
\newcommand{\nuOneHashing}{C_1 \sqrt{\epsilon} \min \left\{ \frac{\log(E/\epsilon)}{\log(1/\delta)}, \sqrt{\frac{\log(E)}{\log(1/\delta)}} \right\}}
\newcommand{\nuSHashing}{C_{\nu} \sqrt{\epsilon s}  \min \left\{ \frac{\log(E/\epsilon)}{\log(1/\delta)}, \sqrt{\frac{\log(E)}{\log(1/\delta)}} \right\}} 
\newcommand{\muASHashing}{\sqrt{s} C_{\nu} C_1^{-1} \muBarEpsDelta}
\newcommand{\muASHashingVariant}{\sqrt{s}\muBarEpsDelta}
\newcommand{\EUpperSHashing}{C_2^2 \epsilon^2 s[4r + \logDeltaI]^{-1} e^{C_s (C_2 \epsilon s)^{-1} \left[ 4r+\logDeltaI \right]}}
\newcommand{\muLower}{ \sqrt{r/n} + \sqrt{8 \log(n/\delta_1)/n } }
\newcommand{\muLowerNoN}{ \sqrt{r} + \sqrt{8 \log(n/\delta_1) } }
\newcommand{\nLower}{ \frac{ \left( \muLowerNoN  \right)^2}{ 
sC_{\nu}^2C_1^{-2}\bar{\mu}(\epsilon,\delta)^2 }}
\newcommand{\nLowerSVariant}{ \frac{ \left( \muLowerNoN  \right)^2}{ s\bar{\mu}(\epsilon,\delta)^2 } }
\newcommand{\mLower}{E C_2^{-2} \epsilon^{-2} \fourRplusLog}
\newcommand{\epsilonPrimeFactorA}{ \frac{1+2\gamma-\gamma^2}{(1-\gamma)(1-\gamma^2)}}
\newcommand{\epsilonPrimeFactor}{\frac{(1-\gamma)(1-\gamma^2)}{1+2\gamma-\gamma^2}}
\renewcommand{\k}{p}
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\yPlus}{Y_+}
\newcommand{\yMinus}{Y_-}
\newcommand{\nPlus}{N_+}
\newcommand{\nMinus}{N_-}
\newcommand{\yPlusExpression}{\set{y_1 + y_2: y_1,y_2 \in Y}}
\newcommand{\yMinusExpression}{\set{y_1 - y_2: y_1,y_2 \in Y}}
\newcommand{\nPlusExpression}{\set{y_i + y_j: i,j \in \left[1,|N|\right]}}
\newcommand{\nMinusExpression}{\set{y_i - y_j: i,j  \in \left[1,|N|\right]}}
\newcommand{\union}[2]{#1\cup#2}
\newcommand{\yExpression}{\set{y_1, y_2, \dots y_{|Y|}}}
\newcommand{\probability}[1]{\P \left( #1 \right)}
\renewcommand{\complement}[1]{\left( #1 \right)^c}
\newcommand{\squareBracket}[1]{\left[ #1 \right]}
\newcommand{\unionNPlusNMinusSetDiffZero}{\union{\nPlus}{ ( \nMinus \setminus \set{0}) }}
\newcommand{\cardinalityNPlus}{\frac{(|N|+1)|N|}{2}}
\newcommand{\cardinalityNMinus}{\frac{(|N|-1)|N|}{2}}
\newcommand{\nMinusSetDiffZero}{\nMinus \setminus \set{0} }
\newcommand{\nMinusOneExpression}{\set{y_i-y_j: 1\leq i <j \leq |N|}}
\newcommand{\nMinusTwoExpression}{\set{y_i - y_j: 1\leq j <i \leq |N|}}
\newcommand{\nMinusOne}{N_-^{(1)}}
\newcommand{\nMinusTwo}{N_-^{(2)}}
\newcommand{\muBarEpsDelta}{\bar{\mu}(\epsilon,\delta)}
\newcommand{\EUpperHashing}{\frac{2 e^{4r}}{\left[ 4r + \logDeltaI \right]\delta }}
\newcommand{\muHatSEpsDelta}{\hat{\mu}(s,\epsilon,\delta)}
\newcommand{\HRHTProb}{1-\delta-\delta_1 + \delta\delta_1}
\newcommand{\bracket}[1]{\left( #1\right)}
\newcommand{\ntsUpperTwo}{\frac{f(x_0)-f^*}{h \bracket{\epsilon, \alphaMin}}}
\newcommand{\ntsUpperTwoGammaC}{\frac{\fZeroMinusfStar}{\etaHAlphaLowGammaC}}

\newcommand{\lkHatSHat}{\hat{l}_k \bracket{\sHat}}
\newcommand{\mkHatSHat}{\mKHat{\sHat}}
\newcommand{\oneOverTwoAlphaK}{\frac{1}{2\alphaK}}
\newcommand{\oneOverAlphaK}{\frac{1}{\alphaK}}
\newcommand{\SKTransposed}{S_k^T}
\newcommand{\lkHat}[1]{\hat{l}_k \bracket{#1}}
\newcommand{\BMax}{B_{max}}
\newcommand{\sKHat}{\hat{s}_k}
\newcommand{\kappaT}{\kappa_T}
\newcommand{\barH}[2]{\bar{h} \bracket{#1,#2}}
\newcommand{\sabs}[1]{\left\lvert #1 \right\rvert}
\newcommand{\halfBMax}{\frac{1}{2}\BMax}
\newcommand{\gradFZetaK}{\grad f \bracket{\zeta_k}}
\newcommand{\SKTransposedsKHat}{S_k^T \sKHat}
\newcommand{\lPlusHalfBmax}{L+\halfBMax}

\newcommand{\deltaOne}{\delta_1}
\newcommand{\logOneOverDeltaOne}{\log \bracket{\frac{1}{\deltaOne}}}
\newcommand{\deltaTwo}{\delta_2}
\newcommand{\logOneOverDeltaTwo}{\log \bracket{\frac{1}{\deltaTwo}}}
\newcommand{\eToQRxSqaured}{e^{q \normTwo{Rx}^2}}
\newcommand{\eToQRySqaured}{e^{q \normTwo{Ry}^2}}
\newcommand{\eToQLOneMinusEps}{e^{ql(1-\epS)}}
\newcommand{\eToMinusQLOneMinusEps}{e^{-ql(1-\epS)}}
\newcommand{\texteq}[1]{\text{\quad #1}}
\newcommand{\lambdaMin}[1]{\lambda_{min} \bracket{#1}}
\newcommand{\lambdaMax}[1]{\lambda_{max} \bracket{#1}}
\newcommand{\muMin}{\mu_{min}}
\newcommand{\muMax}{\mu_{max}}
\newcommand{\tS}{\tilde{S}}
\newcommand{\zK}{z^{k}}
\newcommand{\aZeroOne}{A_0^{(1)}}
\newcommand{\aZeroTwo}{A_0^{(2)}}
\newcommand{\logOneOverDeltaSOne}{\log \bracket{\frac{1}{\deltaSOne}}}
\newcommand{\normInf}[1]{\|#1\|_{\infty}}
\newcommand{\oneOverTwoAlphaMax}{\frac{1}{2\alphaMax}}
\newcommand{\deq}{\mathrel{\mathop:}=}
\newcommand{\fStar}{f^*}
\newcommand{\minGradientM}{\minGradient{M}}
\newcommand{\logOneOverDeltaSTwo}{\log\bracket{1/\deltaSTwo}}
\newcommand{\mkHatSkHat}{\hat{m}_k\bracket{\hat{s}_k}}
\newcommand{\gK}{g_k}
\newcommand{\mK}[1]{m_k \bracket{#1}}
\newcommand{\deltaS}{\delta_S}
\newcommand{\integral}[3]{\int_{#1}^{#2} #3}
\newcommand{\probNEpsGrN}{\probability{\nEps >M}dM}
\newcommand{\kappaEG}{\kappa_{eg}}
\newcommand{\kappaEF}{\kappa_{ef}}
\newcommand{\twoKappa}{(\kappaEG, \kappaEF)}



% Sentence Macros
% \newcommand{\reply}[1]{{\color{blue}#1} \color{black}}
\newcommand{\reply}[1]{#1}
\newcommand{\todo}[1]{{\color{blue}TODO: #1} \color{black}}
\newcommand{\CorTwoDeltaOne}{Suppose \eqref{eqn::deltaSConditionThmTwo} hold and let $\delta_1 \in (0,1)$ satisfy \eqref{eqn:tmp32}}
\newcommand{\IterKTrueandSuccssfulWithAlphaKGeqAlphaMin}{\substack{ \text{Iteration $k$ is true and successful} \\ \text{with $\alphaK \geq \alphaZero \gammaOne^{c+\newL}$}}}
\newcommand{\ThmOneAssumptions}{Let \autoref{AA2}, \autoref{AA3}(i), \autoref{AA4} and \autoref{AA5} hold with $\delta_S \in (0,1), \alphaLow>0$ and $h: \R^2 \to \R$}
\newcommand{\ThmOneDefinitions}{Let $\epsilon>0$, $\nEps$ be defined in \autoref{tab:it::count}, and $f^*$ be defined in \eqref{eqn::fStar} and $C_1$, $C_2$ be defined as 
		\begin{align}
		C_1 &= \frac{1}{\logOneOverGammaOne}\logAlphaZeroOverAlphaLow
		, \label{eqn::C1} \\
		C_2 &= \frac{\log(\gamma_2)}{\logOneOverGammaOne} \label{eqn::C2},
		\end{align}
		where $\alpha_0, \gamma_1, \gamma_2$ are defined in \autoref{alg:generic}
		}
\newcommand{\ThmOneFurtherAssumptions}{Suppose 
\begin{equation}
    1-\delta_S > \frac{C_2}{1+C_2}. \label{eq::delta_S_condition}
\end{equation}}
\newcommand{\ThmOneDeltaOneCondition}{(1-\delta_S)(1-\delta_1) > \frac{C_2}{1+C_2}}
\newcommand{\ThmOneForAnyDeltaOneSuchThat}{for any $\delta_1 \in (0,1)$ with 
\begin{equation}
    \ThmOneDeltaOneCondition,
\end{equation}
}
\newcommand{\defineDOneDTwoDThree}{ 
\begin{align}
    &D_1 = \nPreFactor (f(x_0) - f^*), \label{eqn::D_1}\\
    &D_2 = \nPreFactor \frac{C_1}{1+C_2}, \label{eqn::D_2}\\
    &D_3 = \frac{\delta_1^2}{2}(1-\delta_S). \label{eqn::D_3}
\end{align}
}
\newcommand{\CorOneDefinitions}{Let $f^*$ be defined in \eqref{eqn::fStar}}
\newcommand{\CorOneDeltaOne}{Suppose \eqref{eq::delta_S_condition} holds and let $\delta_1 \in (0,1)$ satisfy \eqref{eqn::deltaOneDeltaSCondition}}
\newcommand{\DOneDTwoDThreeQDefined}{$D_1, D_2, D_3, q$ are defined in \eqref{eqn::D_1}, \eqref{eqn::D_2}, \eqref{eqn::D_3} and \eqref{eqn::q}}
\newcommand{\lemmaThreeAssumptions}{Let \autoref{AA3}(i), \autoref{AA4} and \autoref{AA5} hold with $h: \R^2 \to \R, \alphaLow>0$}
\newcommand{\lemmaThreeSecondSentence}{Let $\epsilon>0, N\in \N$; and $\nEps, \nts$ be defined in \eqref{eqn::nEps} and \autoref{tab:it::count} respectively}
\newcommand{\constantsDescription}{problem-independent constants}
\newcommand{\whereMuBarIsDefined}{where $\muBarEpsDelta$ is defined in \eqref{A:mu-1}}
\newcommand{\theoremFiveFirstSentence}{Suppose that $\epsilon,\delta \in (0,1)$, $r \leq d \leq n, m\leq n \in \N$, $E >0$ satisfy }
\newcommand{\theoremThreeFirstSentence}{Let  $C_1, C_2, C_3, C_M, C_{\nu}, C_s >0$ be \constantsDescription. Suppose that $\epsilon,\delta \in (0, C_3)$, 
$m,\,s\in \N^+$ and $E>0$ satisfy }
\newcommand{\sHS}{S_h(s)}
\newcommand{\anSHashingMat}{an $s$-hashing matrix}
\newcommand{\anSHashingVariantMat}{an $s$-hashing variant matrix}
\newcommand{\refAlgOne}{Algorithm \ref{alg1}}
\newcommand{\solverName}{Ski-LLS}
\newcommand{\solverNameDense}{Ski-LLS-dense}
\newcommand{\solverNameSparse}{Ski-LLS-sparse}
\newcommand{\calibrationDenseCaptionSentenceOne}[1]{Runtime of #1 on dense matrices $A \in \R^{n \times d}$ from Test Set 1
%(defined in \eqref{eq::A_co_dense}, \eqref{eq::A_semi_dense}, \eqref{eq::A_inco_dense}) 
with $n=50000, d=4000$ and $n=50000, d=7000$ and different values of $\gamma=m/d$} 
\newcommand{\calibrationDenseCaptionSentenceTwo}[1]{For each plot, #1 is run three times on (the same) randomly generated $A$. We see that the runtime has low variance despite the randomness in the solver} 
\newcommand{\calibrationDenseCaptionSentenceThree}[1]{We choose #1 to approximately minimize the runtime across the above plots}
\newcommand{\performanceProfileCaption}[1]{Performance profile comparison of \solverName{} with LSRN, LS\_HSL and LS\_SPQR for all matrices $A\in\R^{n\times d}$ in the Florida matrix collection with #1}
\newcommand{\defDenseTestMatrices}{\eqref{eq::A_co_dense}, \eqref{eq::A_semi_dense}, \eqref{eq::A_inco_dense}}

% Figure macros
\newcommand{\calibrationSixFigures}[8]{
\begin{figure}[H]
    \centering
    \begin{minipage}{\mysize\textwidth}
        \centering
        \includegraphics[width=\textwidth]{#1} % first figure itself
    \end{minipage}
    \begin{minipage}{\mysize\textwidth}
        \centering
        \includegraphics[width=\textwidth]{#2} % second figure itself
    \end{minipage}
    \begin{minipage}{\mysize\textwidth}
        \centering
        \includegraphics[width=\textwidth]{#3} % second figure itself
    \end{minipage}    
    \centering
    \begin{minipage}{\mysize\textwidth}
        \centering
        \includegraphics[width=\textwidth]{#4} % first figure itself
    \end{minipage}
    \begin{minipage}{\mysize\textwidth}
        \centering
        \includegraphics[width=\textwidth]{#5} % second figure itself
    \end{minipage}
    \begin{minipage}{\mysize\textwidth}
        \centering
        \includegraphics[width=\textwidth]{#6} % second figure itself
    \end{minipage}        
    \caption{#7} \label{#8}
\end{figure}
}
\newcommand{\threeFigures}[9]{
\begin{figure}
    \begin{minipage}{\mysize\textwidth}
    \centering
        \includegraphics[width=\textwidth]{#1} % first figure itself
        \caption{#2}
        \label{#3}
    \end{minipage}\hfill
    \begin{minipage}{\mysize\textwidth}
    \centering
        \includegraphics[width=\textwidth]{#4} % second figure itself
        \caption{#5}
        \label{#6}
    \end{minipage}
    \begin{minipage}{\mysize\textwidth}
    \centering
        \includegraphics[width=\textwidth]{#7} % third figure itself
        \caption{#8}
        \label{#9}
    \end{minipage}    
\end{figure}
}

\newcommand{\twoFigures}[6]{
    \begin{figure}
    \centering
    \begin{minipage}{\mysize\textwidth}
        \centering
        \includegraphics[width=\textwidth]{#1} % first figure itself
        \caption{#2}
        \label{#3}
    \end{minipage}\hfill
    \begin{minipage}{\mysize\textwidth}
    \centering
    \includegraphics[width=\textwidth]{#4}
    \caption{#5}
    \label{#6}
    \end{minipage}
    \end{figure}
}

% Latex text macros
\newcommand{\mathInTitle}[1]{\texorpdfstring{#1}{TEXT}}
\newcommand{\highlight}[1]{\textcolor{red}{#1} }
\newcommand{\answer}[1]{\textcolor{blue}{#1} }
\newcommand{\singleQuote}[1]{\lq #1\rq}




